A Rigorous Analysis of AODV and its Variants

In this paper we present a rigorous analysis of the Ad hoc On-Demand Distance Vector (AODV) routing protocol using a formal specification in AWN (Algebra for Wireless Networks), a process algebra which has been specifically tailored for the modelling of Mobile Ad Hoc Networks and Wireless Mesh Network protocols. Our formalisation models the exact details of the core functionality of AODV, such as route discovery, route maintenance and error handling. We demonstrate how AWN can be used to reason about critical protocol correctness properties by providing a detailed proof of loop freedom. In contrast to evaluations using simulation or other formal methods such as model checking, our proof is generic and holds for any possible network scenario in terms of network topology, node mobility, traffic pattern, etc. A key contribution of this paper is the demonstration of how the reasoning and proofs can relatively easily be adapted to protocol variants.

==> fig/ex_mswimSect52b_1.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(6.0,0.0){0.28}{d}
   \rput(6.0,0.091){\small$D$}
   \rput(6.0,-0.14){\tiny $1$}
\rput(6.0,0.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \cnode(1.936,-0.5){0.28}{t}
   \rput(1.936,-0.40900000000000003){\small$T$}
   \rput(1.936,-0.64){\tiny $1$}
\rput(1.936,-1.0){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \cnode(1.936,0.5){0.28}{s}
   \rput(1.936,0.591){\small$S$}
   \rput(1.936,0.36){\tiny $1$}
\rput(1.936,1.0){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \cnode(4.0,0.0){0.28}{a}
   \rput(4.0,0.091){\small$A$}
   \rput(4.0,-0.14){\tiny $1$}
\rput(4.0,0.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}

%%  EDGES  %%
   \ncline{s}{a}
   \ncline{t}{a}
   \ncline{a}{d}

%%  MSGS  %%

\endpspicture


==> fig/ex_mswimSect52b_2.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(6.0,0.0){0.28}{d}
   \rput(6.0,0.091){\small$D$}
   \rput(6.0,-0.14){\tiny $1$}
\rput(6.0,0.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \cnode(1.936,-0.5){0.28}{t}
   \rput(1.936,-0.40900000000000003){\small$T$}
   \rput(1.936,-0.64){\tiny $1$}
\rput(1.936,-1.0){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \cnode(1.936,0.5){0.28}{s}
   \rput(1.936,0.591){\small$S$}
   \rput(1.936,0.36){\tiny $2$}
\rput(1.936,1.0){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \cnode(4.0,0.0){0.28}{a}
   \rput(4.0,0.091){\small$A$}
   \rput(4.0,-0.14){\tiny $1$}
\rput(4.0,0.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (S & 2 & \mbox{val} & 1 & S)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{s}{a}
   \ncline{t}{a}
   \ncline{a}{d}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{->}{s}{a}
   \aput[1pt]{:U}{\tiny \msg{RREQ}{s}{d}~~}

\endpspicture


==> fig/ex_mswimSect52b_3.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(6.0,0.0){0.28}{d}
   \rput(6.0,0.091){\small$D$}
   \rput(6.0,-0.14){\tiny $1$}
\rput(6.0,0.5){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \cnode(1.936,-0.5){0.28}{t}
   \rput(1.936,-0.40900000000000003){\small$T$}
   \rput(1.936,-0.64){\tiny $2$}
\rput(1.936,-1.0){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \cnode(1.936,0.5){0.28}{s}
   \rput(1.936,0.591){\small$S$}
   \rput(1.936,0.36){\tiny $2$}
\rput(1.936,1.0){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
   \end{array}$}

}
   \cnode(4.0,0.0){0.28}{a}
   \rput(4.0,0.091){\small$A$}
   \rput(4.0,-0.14){\tiny $1$}
\rput(4.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (S & 2 & \mbox{val} & 1 & S)\\
       (T & 2 & \mbox{val} & 1 & T)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{s}{a}
   \ncline{t}{a}
   \ncline{a}{d}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{<-}{a}{t}
   \aput[1pt]{:D}{\tiny \msg{RREQ}{t}{d}~~}

\endpspicture


==> fig/ex_mswimSect52b_4.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(6.0,0.0){0.28}{d}
   \rput(6.0,0.091){\small$D$}
   \rput(6.0,-0.14){\tiny $1$}
\rput(6.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (S & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(1.936,-0.5){0.28}{t}
   \rput(1.936,-0.40900000000000003){\small$T$}
   \rput(1.936,-0.64){\tiny $2$}
\rput(1.936,-1.105){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (S & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(1.936,0.5){0.28}{s}
   \rput(1.936,0.591){\small$S$}
   \rput(1.936,0.36){\tiny $2$}
\rput(1.936,1.0){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
   \end{array}$}

}
   \cnode(4.0,0.0){0.28}{a}
   \rput(4.0,0.091){\small$A$}
   \rput(4.0,-0.14){\tiny $1$}
\rput(4.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (S & 2 & \mbox{val} & 1 & S)\\
       (T & 2 & \mbox{val} & 1 & T)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{s}{a}
   \ncline{t}{a}
   \ncline{a}{d}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{->}{a}{d}
   \aput[1pt]{:U}{\tiny \msg{RREQ}{s}{d}~~}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{->}{a}{t}
   \aput[1pt]{:D}{\tiny ~~\msg{RREQ}{s}{d}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{<-}{s}{a}
   \aput[1pt]{:U}{\tiny ~~\msg{RREQ}{s}{d}}

\endpspicture


==> fig/ex_mswimSect52b_5.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(6.0,0.0){0.28}{d}
   \rput(6.0,0.091){\small$D$}
   \rput(6.0,-0.14){\tiny $1$}
\rput(6.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (S & 2 & \mbox{val} & 2 & A)\\
       (T & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(1.936,-0.5){0.28}{t}
   \rput(1.936,-0.40900000000000003){\small$T$}
   \rput(1.936,-0.64){\tiny $2$}
\rput(1.936,-1.105){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (S & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(1.936,0.5){0.28}{s}
   \rput(1.936,0.591){\small$S$}
   \rput(1.936,0.36){\tiny $2$}
\rput(1.936,1.105){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (T & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(4.0,0.0){0.28}{a}
   \rput(4.0,0.091){\small$A$}
   \rput(4.0,-0.14){\tiny $1$}
\rput(4.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (S & 2 & \mbox{val} & 1 & S)\\
       (T & 2 & \mbox{val} & 1 & T)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{s}{a}
   \ncline{t}{a}
   \ncline{a}{d}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{->}{a}{t}
   \aput[1pt]{:D}{\tiny ~~\msg{RREQ}{t}{d}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{<-}{s}{a}
   \aput[1pt]{:U}{\tiny ~~\msg{RREQ}{t}{d}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{->}{a}{d}
   \aput[1pt]{:U}{\tiny \msg{RREQ}{t}{d}~~}

\endpspicture


==> fig/ex_mswimSect52b_6.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(6.0,0.0){0.28}{d}
   \rput(6.0,0.091){\small$D$}
   \rput(6.0,-0.14){\tiny $1$}
\rput(6.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (S & 2 & \mbox{val} & 2 & A)\\
       (T & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(1.936,-0.5){0.28}{t}
   \rput(1.936,-0.40900000000000003){\small$T$}
   \rput(1.936,-0.64){\tiny $2$}
\rput(1.936,-1.105){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (S & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(1.936,0.5){0.28}{s}
   \rput(1.936,0.591){\small$S$}
   \rput(1.936,0.36){\tiny $2$}
\rput(1.936,1.21){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (D & 1 & \mbox{val} & 2 & A)\\
       (T & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(4.0,0.0){0.28}{a}
   \rput(4.0,0.091){\small$A$}
   \rput(4.0,-0.14){\tiny $1$}
\rput(4.0,0.71){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 1 & \mbox{val} & 1 & D)\\
       (S & 2 & \mbox{val} & 1 & S)\\
       (T & 2 & \mbox{val} & 1 & T)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{s}{a}
   \ncline{t}{a}
   \ncline{a}{d}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{<-}{a}{d}
   \aput[1pt]{:U}{\tiny ~~\msg{RREP}{s}{d}}
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{<-}{s}{a}
   \aput[1pt]{:U}{\tiny ~~\msg{RREP}{s}{d}}

\endpspicture


==> fig/ex_mswimSect52b_7.tex <==
%% Latex Commands%%
\newcommand{\msg}[3]{#1${}_{\!\!\;\MakeUppercase{#2}\!\!\:\shortrightarrow\!\MakeUppercase{#3}}$}
\newcommand{\msgerr}{RERR}
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(6.0,0.0){0.28}{d}
   \rput(6.0,0.091){\small$D$}
   \rput(6.0,-0.14){\tiny $1$}
\rput(6.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (S & 2 & \mbox{val} & 2 & A)\\
       (T & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(1.936,-0.5){0.28}{t}
   \rput(1.936,-0.40900000000000003){\small$T$}
   \rput(1.936,-0.64){\tiny $2$}
\rput(1.936,-1.105){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (S & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(1.936,0.5){0.28}{s}
   \rput(1.936,0.591){\small$S$}
   \rput(1.936,0.36){\tiny $2$}
\rput(1.936,1.21){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (D & 1 & \mbox{val} & 2 & A)\\
       (T & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}
   \cnode(4.0,0.0){0.28}{a}
   \rput(4.0,0.091){\small$A$}
   \rput(4.0,-0.14){\tiny $1$}
\rput(4.0,0.71){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & 1 & \mbox{val} & 1 & D)\\
       (S & 2 & \mbox{val} & 1 & S)\\
       (T & 2 & \mbox{val} & 1 & T)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline{s}{a}
   \ncline{t}{a}
   \ncline{a}{d}

%%  MSGS  %%
   \ncline[linewidth=0.8pt,linecolor=red,arrowsize=4pt,offset=0pt]{<-}{a}{d}
   \aput[1pt]{:U}{\tiny ~~\msg{RREP}{t}{d}}

\endpspicture


==> fig/ex_sqn_up.tex <==
\pspicture(-10,-10)(10,10)

%%  NODES  %%
   \cnode(2.0,0.0){0.28}{s}
   \rput(2.0,0.091){$S$}
   \rput(2.0,-0.14){\tiny $2$}
   \rput(2.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{inv} & 1 & A)\\
       (D & {\bf 2} & \mbox{inv} & 2 & A)\\
   \end{array}$}

}
   \cnode(4.0,0.0){0.28}{a}
   \rput(4.0,0.091){$A$}
   \rput(4.0,-0.14){\tiny $1$}
   \rput(4.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (D & {\bf 1} & \mbox{val} & 1 & D)\\
       (S & 2 & \mbox{val} & 1 & S)\\
   \end{array}$}

}
   \cnode(6.0,0.0){0.28}{d}
   \rput(6.0,0.091){$D$}
   \rput(6.0,-0.14){\tiny $1$}
   \rput(6.0,0.605){
   {\tiny$\begin{array}{l@{,}r@{,}c@{,}r@{,}r}
       (A & 0 & \mbox{val} & 1 & A)\\
       (S & 2 & \mbox{val} & 2 & A)\\
   \end{array}$}

}

%%  EDGES  %%
   \ncline[linestyle=dashed]{s}{a}
   \ncline{a}{d}

%%  MSGS  %%

\endpspicture

